A Type System for Tom

Extending a given language with new dedicated features is a general and quite used approach to make the programming language more adapted to problems. Being closer to the application, this leads to less programming flaws and easier maintenance. But of course one would still like to perform program analysis on these kinds of extended languages, in particular type checking and inference. In this case one has to make the typing of the extended features compatible with the ones in the starting language. The Tom programming language is a typical example of such a situation as it consists of an extension of Java that adds pattern matching, more particularly associative pattern matching, and reduction strategies. This paper presents a type system with subtyping for Tom, that is compatible with Java's type system, and that performs both type checking and type inference. We propose an algorithm that checks if all patterns of a Tom program are well-typed. In addition, we propose an algorithm based on equality and subtyping constraints that infers types of variables occurring in a pattern. Both algorithms are exemplified and the proposed type system is showed to be sound and complete.

==> eptcsdata.tex <==
\providecommand{\event}{I. Mackie and A. Martins Moreira (Eds.): Tenth International\\Workshop on Rule-Based Programming (RULE 2009)}
\providecommand{\volume}{21}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{51}
\providecommand{\eid}{5}

